Enabling Efficient Wearables: An Analysis of Low-Power Microcontrollers for Biomedical Applications

Breakthroughs in ultra-low-power chip technology are transforming biomedical wearables, making it possible to monitor patients in real time with devices operating on mere {\mu}W. Although many studies have examined the power performance of commercial microcontrollers, it remains unclear which ones perform best across diverse application profiles and which hardware features are most crucial for minimizing energy consumption under varying computational loads. Identifying these features for typical wearable applications and understanding their effects on performance and energy efficiency are essential for optimizing deployment strategies and informing future hardware designs. In this work, we conduct an in-depth study of state-of-the-art (SoA) micro-controller units(MCUs) in terms of processing capability and energy efficiency using representative end-to-end SoA wearable applications. We systematically benchmark each platform across three primary application phases: idle, data acquisition, and processing, allowing a holistic assessment of the platform processing capability and overall energy efficiency across varying patient-monitoring application profiles. Our detailed analysis of performance and energy discrepancies across different platforms reveals key strengths and limitations of the current low-power hardware design and pinpoints the strengths and weaknesses of SoA MCUs. We conclude with actionable insights for wearable application designers and hardware engineers, aiming to inform future hardware design improvements and support optimal platform selection for energy-constrained biomedical applications.

==> Acknowledgments.tex <==
\section*{Acknowledgments}
%This should be a simple paragraph before the References to thank those individuals and institutions who have supported your work on this article.

This work was supported in part by the Swiss NSF ML-Edge Project under Grant 200020\_182009, the Swiss NSF ML-Edge Project under Grant 200020\_182009, the ERC Consolidator Grant COMPUSAPIEN (GA No. 725657), and the EC H2020 WiPLASH (GA No. 863337). 



==> notes.tex <==
- Dimitrios, Denisa: why do we choose the applications we choose, and why not others? Why the selection of applications is necessary and sufficient.
-DONE


- Dimitrios, Ruben, and Denisa: show that we use the application metrics to choose the applications in the benchmarks so that they cover all dimensions in the proposed taxonomy. Exemplify metrics measurements for each application in the text to illustrate this.
- mostrar que usamos las metrics, a traves de las metricas


- Denisa: New template!!!
-DONE


- Dimitrios, Denisa: Takeaways - mark them as we get results and conclusions for each analyzed application. Eg. Takeaway1: nr of registers limits # of unrolling
-DONE

- Dimitrios, Denisa: Lessons learned - most important takeaways synthesized in a small section before conclusions

 - Ruben, Dimitrios, Stefano
in 3) SeizDetCNN we say that MAC can take 1,2, or 3 cycles. how do we obtain the #cycles for each platform? experiment, datasheet? Explain it so that the method is replicable! Any conflict between the experimental nr of cycles and the datasheet? An appendix may be necessary, no need for code, just explain in words.
- soft takeaway: need barrel shifter (ok-the evaluated architectures already have it)
- important takeaway: pattern MAC operations in fixed point is very particular. Suggest MAC implementation can be optimized to take advantage of the order of the instructions, using an efficient barrel shifter, etc. 
- missing sin/cos/log
-DONE

Fig4 -\linewidth - done

- Denisa: right align tables w/ numbers

- Denisa: blind review? to put bio notes or not (removed the bionotes) -done

- Ruben: ++ references, tooo few right now
SDK, boards, tools,
- 
-




-"operate in uW range (SmartCardia)" -  look for other platforms/applications as reference instead of smartcards (recent, custom-made, and/or some other from our lab) top right page 1

 - Dimitrios: Table 1- dynamic memory - NA? no data, need of experiments?
